Language Steering for Multilingual In-Context Learning

If multilingual language model representations contain separable language-associated structure, then shifting between languages may require only simple activation-space interventions. To test this hypothesis, we study multilingual in-context learning (ICL) as a controlled setting: few-shot demonstrations are provided in English while the test query is in a target language, creating a clear cross-lingual transfer challenge. We propose language vectors, which are computed as mean activation differences between parallel source and target language examples at a particular layer and applied as inference-time offsets to the model's hidden states. Across three tasks spanning 19 languages and three models, our method improves over English few-shot prompting without any parameter updates. Beyond performance, the vectors encode interpretable linguistic structure: closely related languages form tight clusters, and vectors transfer effectively across tasks and languages, with closely related languages' vectors recovering more of the gain than distant ones. Together, these findings suggest that language occupies structured directions in multilingual activation space, and that inference-time interventions on English demonstrations can narrow the cross-lingual ICL gap.

==> results.tex <==


% \subsection{Datasets used and setup}



% For each dataset, we divide the test set of the data into three parts: train, val and test. The train split is used to compute the steering vector, val split is used to decide the best configuration (layer, position, steering magnitude), test split is used to test the results on the best config chosen from the val set. Apart from this, we use 6-8 datapoints from the training set to be used as few shot examples. 



\subsection{Setup}

% We test on three instruction-tuned models: \textit{\llamamodel, \qwenseven, \qwenfourteen} \cite{grattafiori2024llama,team2024qwen2} and consider three datasets: MGSM (mathematical reasoning) \cite{shi2022language}, MSVAMP (arithmetic word problems) \cite{chen2024breaking} and XNLI (natural language inference) \cite{conneau2018xnli}.

We test on three instruction-tuned models: \llamamodel, \qwenseven, and \qwenfourteen\ \cite{grattafiori2024llama, team2024qwen2}. We consider three datasets: MGSM (mathematical reasoning) \cite{shi2022language}, MSVAMP (arithmetic word problems) \cite{chen2024breaking}, and XNLI (natural language inference) \cite{conneau2018xnli}.




% We evaluate our approach across three instruction-tuned models and three multilingual datasets. For models, we use Llama-3.1-8B-Instruct, Qwen2.5-7B-Instruct, and Qwen2.5-14B-Instruct \cite{}, which are better suited for following the chain-of-thought reasoning patterns in our prompts. We test on three diverse multilingual datasets: MGSM (mathematical reasoning) \cite{shi2022language}, MSVAMP (mathematical reasoning with commonsense elements) \cite{chen2024breaking}, and XNLI (natural language inference) \cite{conneau2018xnli}.

% \textbf{Data Splits.} We partition the test set into three equal parts: compute ($\mathcal{D}_{\text{compute}}$) for steering vector calculation, validation ($\mathcal{D}_{\text{val}}$) for hyperparameter and configuration selection, and test ($\mathcal{D}_{\text{test}}$) for final evaluation. Since some benchmarks 
% provide minimal training data (e.g., MGSM has only 8 training examples), we partition the test set uniformly across all datasets for consistency. We sample 6 examples from the available training data to serve as few-shot 
% demonstrations, kept fixed across all experiments for a given dataset.While per-language hyperparameter selection requires a small validation set, this is a one-time offline cost with no effect on inference. Task-level configurations (Appendix \ref{app:hparam}) offer a practical alternative when per-language validation data is unavailable.

\paragraph{Data Splits.} We partition the test set into three equal parts: compute ($\mathcal{D}_{\text{compute}}$) for steering vector calculation, validation ($\mathcal{D}_{\text{val}}$) for hyperparameter and configuration selection, and test ($\mathcal{D}_{\text{test}}$) for final evaluation. Since training data is minimal or unavailable for some benchmarks, we partition the test set uniformly across all datasets for consistency. We sample 6 examples from the available training data as few-shot demonstrations, kept fixed across all experiments. Task-level configurations (Appendix~\ref{app:hparam}) offer a practical alternative when per-language validation data is unavailable.
 
\paragraph{Implementation Details.}While calculating the vector, we create $N = |\mathcal{D}_{\text{compute}}|$ samples, ensuring each example from the compute set appears at least once across all samples, with remaining slots filled through random sampling with replacement. We use $k=6$ few-shot pairs per sample, mirroring the test-time prompt structure to ensure the steering vector is computed under conditions consistent with inference. We perform a grid search over steering layers $t \in \{5, 10, 15, 20, 25, 30\}$, scaling factors $\alpha \in \{0.5, 1.0, 2.0, 3.0\}$, and the four steering position configurations on $\mathcal{D}_{\text{val}}$. The reported results on $\mathcal{D}_{\text{test}}$ correspond to per-language validation-selected configurations.

% Only configurations achieving validation accuracy above the source baseline are evaluated on $\mathcal{D}_{\text{test}}$. The reported results for \textit{Ours} reflect per-language optimal configurations; 
% hyperparameters may therefore differ across languages.


% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{6pt}
% \small
% \begin{tabular}{lcccc}
% \toprule
% \multirow{2}{*}{Model} & \multicolumn{4}{c}{Performance} \\
% \cmidrule(lr){2-5}
% & B & MFS & Ours & \cellcolor{LightGray!30}OR \\
% \midrule
% \multicolumn{5}{c}{MGSM} \\
% \midrule
%  \llamamodel     
%  & 61.01 & 63.19 & \bf{65.87} & \cellcolor{LightGray!30}68.16 \\
%  \qwenseven         
%  & 68.95 & 69.94 & \bf{71.83} & \cellcolor{LightGray!30}73.21 \\
%  \qwenfourteen     
%  & 81.55 & 82.84 & \bf{84.23} & \cellcolor{LightGray!30}84.72 \\
% \midrule
% \multicolumn{5}{c}{XNLI} \\
% \midrule
%  \llamamodel            
%  & 61.38 & 61.68 & \bf{64.31} & \cellcolor{LightGray!30}65.04  \\
%  \qwenseven      
%  & 74.81 & 73.27 & \bf{75.51} & \cellcolor{LightGray!30}74.53 \\
%  \qwenfourteen      
%  & 72.73 & 73.91 & \bf{74.66} & \cellcolor{LightGray!30}76.45 \\
% \midrule
% \multicolumn{5}{c}{MSVAMP} \\
% \midrule
%  \llamamodel     
%  & 65.84 & \bf{68.66} & {68.60} & \cellcolor{LightGray!30}70.06 \\
%  \qwenseven       
%  & 75.18 & \bf{76.94} & 76.68 & \cellcolor{LightGray!30}77.65 \\
%  \qwenfourteen      
%  & 82.10 & 82.90 & \bf{83.90} & \cellcolor{LightGray!30}83.03 \\
% \bottomrule
% \end{tabular}
% \caption{Average performance comparison across three datasets and three models. B = Baseline, MFS = Multilingual Few-Shot Baseline \cite{tu2025blessing}, OR = Oracle. Oracle is the upper bound and is not for a direct comparison. More details are in Appendix \ref{app:other_models}. \kh{mention detailed results are in appendix X} \kh{Consider make this table as a cross-column table, so the format maps Table 1.}}
% \label{tab:main_results}
% \end{table}

\paragraph{Baselines.} We compare our method against two baselines: (1) \textit{Source baseline (B)}: few-shot prompts with source questions and source chain-of-thought and answer; (2) \textit{Multilingual few-shot (MFS)}: few-shot examples drawn from multiple languages with their respective answers \citet{tu2025blessing}, representing the approach of diversifying few-shot examples across languages. To understand what our upper bound would be when evaluating, we also test: \textit{Oracle}: uses target-language few-shot demonstrations and serves as an upper bound. Following \citet{tu2025blessing}, wherever there is a chain of thought reasoning involved, it's always in the source language (English).



\begin{table*}[t]
\centering
\setlength{\tabcolsep}{6pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{4}{c}{MGSM} & \multicolumn{4}{c}{XNLI} & \multicolumn{4}{c}{MSVAMP} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
& B & MFS & Ours & \cellcolor{LightGray!30}OR
& B & MFS & Ours & \cellcolor{LightGray!30}OR
& B & MFS & Ours & \cellcolor{LightGray!30}OR \\
\midrule
\llamamodel
& 61.01 & 63.19 & \bf{65.87} & \cellcolor{LightGray!30}68.16
& 61.38 & 61.68 & \bf{64.31} & \cellcolor{LightGray!30}65.04
& 65.84 & \bf{68.66} & {68.60} & \cellcolor{LightGray!30}70.06 \\
\qwenseven
& 68.95 & 69.94 & \bf{71.83} & \cellcolor{LightGray!30}73.21
& 74.81 & 73.27 & \bf{75.51} & \cellcolor{LightGray!30}74.53
& 75.18 & \bf{76.94} & 76.68 & \cellcolor{LightGray!30}77.65 \\
\qwenfourteen
& 81.55 & 82.84 & \bf{84.23} & \cellcolor{LightGray!30}84.72
& 72.73 & 73.91 & \bf{74.66} & \cellcolor{LightGray!30}76.45
& 82.10 & 82.90 & \bf{83.90} & \cellcolor{LightGray!30}83.03 \\
\bottomrule
\end{tabular}}
\caption{Average performance comparison across three datasets and three models. B = Baseline, MFS = Multilingual Few-Shot Baseline \cite{tu2025blessing}, OR = Oracle. Oracle is the upper bound and is not for a direct comparison. Detailed per-language results are in Appendix~\ref{app:other_models}.}
\label{tab:main_results}
\end{table*}


% Wherever there are few shots involved, we use an English chain-of-thought reasoning, with the question in the target language.\cite{shi2022language} 


% and English chain-of-thought, representing an upper bound on performance without steering, as English chain-of-thought reasoning is typically of higher quality than target language reasoning.

% \textbf{Few-Shot Prompt Structure.} During evaluation, our prompt contains few-shot questions in the source language (English) with answer explanations and the final answer. The question to be answered is in the target language. We steer some part of this prompt to understand whether that can help the model change the mode from English to the target language while processing the given question. For our tasks, which are reasoning and inference-based, the final answer remains the same across languages.



\subsection{Results}

\paragraph{Performance on Llama Model.}
Detailed accuracy results on $\mathcal{D}_{\text{test}}$ for the \llamamodel\ model are shown in 
Table~\ref{tab:multi_detailed} across the three datasets, covering 19 languages. Our method 
improves over the source baseline (B) across most languages and datasets, demonstrating that 
activation steering enables effective cross-lingual transfer without any parameter updates. 
MGSM shows the most consistent and substantial improvements, indicating that structured 
mathematical reasoning particularly benefits from cross-lingual steering. On MSVAMP, our 
method performs comparably to MFS, with differences of less than 0.3 points on average. 
XNLI presents the most mixed results: gains vary considerably across languages, and MFS 
occasionally outperforms ours. Overall, our method shows the strongest gains on reasoning 
tasks, remains competitive with MFS on MSVAMP, and provides consistent improvements 
over the source baseline across settings.

\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccc}
\toprule
\textbf{Language} & \textbf{MGSM} & \textbf{MSVAMP} & \textbf{XNLI} \\
\midrule
Arabic     & ---    & ---    & 10/3.0 \\
Basque     & 5/1.0  & ---    & ---    \\
Bengali    & 20/1.0 & 5/0.5  & ---    \\
Bulgarian  & ---    & ---    & 10/3.0 \\
Catalan    & 20/3.0 & ---    & ---    \\
Chinese    & 30/0.5 & 5/0.5  & 5/3.0  \\
French     & 5/1.0  & 15/0.5 & 10/3.0 \\
Galician   & 5/1.0  & ---    & ---    \\
German     & 5/2.0  & 30/1.0 & 5/3.0  \\
Greek      & ---    & ---    & 10/3.0 \\
Hindi      & ---    & ---    & 10/3.0 \\
Japanese   & 5/1.0  & 10/0.5 & ---    \\
Russian    & 30/0.5 & 25/0.5 & 10/3.0 \\
Spanish    & 30/1.0 & 5/0.5  & 10/3.0 \\
Swahili    & 5/1.0  & 5/0.5  & 5/3.0  \\
Thai       & 5/0.5  & 5/2.0  & 10/3.0 \\
Turkish    & ---    & ---    & 10/3.0 \\
Urdu       & ---    & ---    & 10/3.0 \\
Vietnamese & ---    & ---    & 10/3.0 \\
\bottomrule
\end{tabular}
\caption{Best layer/$\alpha$ per language and task for \llamamodel. Each cell shows \textit{layer}/$\alpha$; {---} indicates the language was not evaluated on that task.}

\paragraph{Performance on Other Models.}
Table~\ref{tab:main_results} summarizes average performance across all languages for each 
model and dataset combination. Our method consistently outperforms the source baseline on 
MGSM across all three models, with improvements ranging from 2.9\% to 5.4\%, confirming 
that activation steering is especially effective for structured mathematical reasoning. On 
XNLI and MSVAMP, improvements are generally smaller, with MFS remaining competitive 
especially on MSVAMP. Despite this, our method performs comparably to or better than the 
baselines in the majority of cases across models and datasets. Per-language results for 
\qwenseven\ and \qwenfourteen\ are in Appendix~\ref{app:other_models}.

\paragraph{Optimal Layer and $\alpha$.}
Table~\ref{tab:best_performing_layers} reports the optimal steering layer and scaling factor 
$\alpha$ per language and task for \llamamodel. For XNLI, layer 10 dominates across 11 out 
of 14 languages, consistent with middle-layer representations encoding semantic and pragmatic 
features relevant to natural language inference. For MGSM and MSVAMP, layer 5 is most 
frequent (7/12 and 5/9 languages respectively), suggesting mathematical reasoning benefits 
from steering at earlier layers where surface-level language features are more prominent. 
The optimal $\alpha$ also varies: $\alpha = 3.0$ dominates for XNLI while MGSM and MSVAMP 
show lower optimal values, suggesting natural language inference requires stronger steering 
than structured reasoning tasks. Task-level configurations in Appendix~\ref{app:hparam} 
remain consistently above the source baseline, confirming the method is effective without 
per-language validation data.

\paragraph{Steering Position.}
Table~\ref{tab:intervention_detailed} shows accuracy across the four steering position 
configurations on MGSM. No single position dominates across all languages. On average, 
steering on the few-shot demonstrations (\texttt{on\_fewshot}) achieves the highest accuracy 
(65.58\%), roughly a 4-point improvement over baseline, likely because the model forms its 
task understanding while processing the demonstrations. In the absence of validation data, 
\texttt{on\_fewshot} is the recommended default given its consistently strong average 
performance.

Detailed accuracy results on $\mathcal{D}_{\text{test}}$ for the \llamamodel\ model are shown in Table \ref{tab:multi_detailed} across the three datasets. We test on a total of 19 languages across the datasets. For every language, we report accuracy under two baselines: the source-language few-shot baseline and the multilingual few-shot method \cite{tu2025blessing}.
% We can see that our method (RFS) consistently outperforms the baselines. 


% Results on the test set are shown in Table \ref{tab:multi_detailed} for the Llama3.1-8b-instruct model across the three datasets. We test on a total of 19 languages. We can see that our method (RFS) consistently improves from the baseline with a few exceptions. For certain languages, RFS also beats the upper bound. 

% A closer examination reveals several noteworthy patterns. First, steering effectiveness varies substantially across languages, with improvements ranging from modest gains (e.g., Bengali on MGSM: 4.76\% over baseline) to significant boosts (e.g., Galician on MGSM: 9.52\% over baseline). Second, the instances where RFS surpasses the Oracle baseline are particularly interesting for example, Basque on MGSM (36.90\% vs. 52.38\%) and Bengali on XNLI (61.90\% vs. 58.33\%) suggesting that steering can sometimes enable more effective cross-lingual transfer than simply providing target language demonstrations. This may occur when the steering vector successfully bridges representational gaps while preserving the model's stronger English reasoning capabilities. Third, performance improvements are generally more consistent on MGSM and MSVAMP compared to XNLI, potentially because mathematical reasoning benefits more from structured cross-lingual transfer than natural language inference tasks. Languages with larger script differences from English (e.g., Thai, Bengali, Japanese) show varied results, indicating that steering effectiveness depends on factors beyond surface-level orthographic similarity. Finally, the multilingual few-shot baseline (BL) sometimes outperforms our method (e.g., Chinese on XNLI: 61.38\% vs. 59.28\%), highlighting that strategic few-shot selection remains a competitive approach, though our steering method achieves superior results in the majority of cases.

% Overall, RFS improves over the source baseline (B) for the majority of languages and datasets, demonstrating that activation steering is an effective mechanism for cross-lingual transfer without modifying model parameters or prompts. The magnitude of gains varies across languages, indicating that steering effectiveness is language-dependent rather than uniform.

% Dataset-wise trends reveal clear differences. On MGSM, RFS yields the most consistent and substantial improvements, suggesting that structured mathematical reasoning benefits strongly from cross-lingual steering. On MSVAMP, the multilingual few-shot baseline (BL) is comparatively stronger and remains competitive for several languages, highlighting the effectiveness of diverse demonstrations for arithmetic word problems; nevertheless, RFS still achieves higher accuracy in many cases. In contrast, results on XNLI are more mixed, with gains varying across languages and BL occasionally outperforming RFS, reflecting the greater linguistic and semantic variability inherent in natural language inference. Taken together, these results show that RFS provides a robust and complementary alternative to multilingual few-shot prompting, with particularly strong benefits on reasoning-centric tasks.
Our method improves over the source baseline (B) across most languages and datasets, demonstrating that activation steering enables effective cross-lingual transfer without any parameter updates. Clear patterns emerge across datasets. MGSM shows the most consistent and substantial improvements, indicating that structured mathematical reasoning particularly benefits from cross-lingual steering. On MSVAMP, our method performs comparably to MFS, with differences of less than 0.3 points on average, suggesting that for arithmetic word problems, diverse demonstrations provide a similarly effective steering signal to activation-based intervention.
% On MSVAMP, the multilingual few-shot baseline (MFS) proves more competitive, often matching or slightly exceeding our method, which reflects the value of diverse demonstrations for arithmetic word problems. 
% XNLI presents the most mixed results: gains vary considerably across languages, and MFS occasionally outperforms ours.
% % ikely due to the greater linguistic and semantic variability in natural language inference tasks. 
% Overall, these findings show that our method provides a complementary approach to MFS.
XNLI presents the most mixed results: gains vary considerably across languages, and MFS occasionally outperforms ours. Overall, our method shows the strongest gains on reasoning tasks, remains competitive with MFS on MSVAMP, and provides consistent improvements over the source baseline across settings.

\label{tab:best_performing_layers}
\end{table}
% The varying magnitude of gains across languages suggests that steering effectiveness depends on language-specific characteristics rather than being uniform. This is further 
% supported by our sensitivity analysis (Appendix~\ref{appendix:sensitivity}), 
% which shows that performance is generally stable across compute set sizes, 
% with higher variance for typologically distant languages such as Basque. 

\begin{table}[htp]
\centering
\setlength{\tabcolsep}{7pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
Language & B & OF & AF & OQ & ENT \\
\midrule
Bengali & 57.14 & 60.71 & \bf{61.90} & 60.71 & 55.95 \\
Catalan & 64.29 & 66.67 & \bf{69.05} & 67.86 & \bf{69.05} \\
German & 66.67 & \bf{75.00} & \textcolor{gray}{--} & 69.05 & 64.29 \\
Spanish & \bf{77.38} & 73.81 & 75.00 & 76.19 & 72.62 \\
Basque & 32.14 & 35.71 & \bf{36.90} & 33.33 & \bf{36.90} \\
French & 61.90 & 67.86 & 64.29 & 67.86 & \bf{70.24} \\
Galician & 64.29 & \bf{73.81} & 69.05 & 66.67 & \bf{73.81} \\
Japanese & \bf{55.95} & \textcolor{gray}{--} & \bf{55.95} & \textcolor{gray}{--} & \textcolor{gray}{--} \\
Russian & 71.43 & 69.05 & \bf{72.62} & \bf{72.62} & 69.05 \\
Swahili & 55.95 & \bf{65.48} & 60.71 & 63.10 & \bf{65.48} \\
Thai & 57.14 & \bf{61.90} & 54.76 & \bf{61.90} & 59.52 \\
Chinese & 67.86 & \bf{71.43} & \bf{71.43} & \bf{71.43} & \bf{71.43} \\
\midrule
Average & 61.01 & \textbf{65.58} & 62.88 & 64.61 & 64.39 \\

\bottomrule
\end{tabular}}
\caption{Per-language accuracy across steering position configurations for \llamamodel\ on MGSM. B = Baseline, OF = On Few-shot, AF = After Few-shot, OQ = On Question, ENT = Entire Prompt. Dashes indicate configurations where no validation improvement over baseline was found. \textbf{Bold} indicates the best score per language.}
\label{tab:intervention_detailed}
\end{table}



% offers a robust complement to multilingual few-shot prompting, with especially strong advantages for reasoning-heavy tasks.






% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{8pt}
% \small
% \caption{ Cross-task transfer results across all task-vector combinations between MGSM, MSVAMP, and XNLI on Qwen2.5-7b-instruct. For each task pair, we compute steering vectors from one task and evaluate on another task. B-Baseline, MFS - Multilingual few-shot, Our method, CT-Cross-task transfer, OR-Oracle. Results show bidirectional transfer for all language pairs common to both tasks.}

% \begin{tabular}{ccccccccccccc}
% \toprule
% \multicolumn{4}{c}{MGSM (vector) $\rightarrow$ XNLI (eval)} & \multicolumn{4}{c}{MGSM (vector) $\rightarrow$ MSVAMP (eval)} & \multicolumn{4}{c}{XNLI (vector) $\rightarrow$ MSVAMP (eval)} \\
% \cmidrule(lr){1-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12}
%  B & MFS & Ours & CT & B & MFS & Ours & CT & B & MFS & Ours & CT \\
% \midrule
% 75.19 & 74.22 & 75.92 & \bf{75.96} & 75.18 & \bf{76.94} & 76.68 & 75.18 & 73.64 & 74.32 & \bf{76.53} & 76.36 \\
% \midrule
% \midrule
% \multicolumn{4}{c}{XNLI (vector) $\rightarrow$ MGSM (eval)} & \multicolumn{4}{c}{MSVAMP (vector) $\rightarrow$ MGSM (eval)} & \multicolumn{4}{c}{MSVAMP (vector) $\rightarrow$ XNLI (eval)} \\
% \cmidrule(lr){1-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12}
%  B &MFS & Ours & CT & B & MFS & Ours & CT & B & MFS & Ours & CT \\
% \midrule
% 75.18 & \bf{76.94} & 76.68  & 75.83 & 71.69 & 73.54 & \bf{74.34} & 72.22 & 75.19 & 74.22 & \bf{75.92} & \color{red}47.98 \\
% \bottomrule
% \end{tabular}

% \label{tab:cross_task}
% \end{table*}



% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{6pt}
% \small

% \begin{tabular}{lccccc}
% \toprule
% Language & B & OF & AF & OQ & ENT \\
% \midrule
% Bengali & 57.14 & 60.71 & \bf{61.90} & 60.71 & 55.95 \\
% Catalan & 64.29 & 66.67 & \bf{69.05} & 67.86 & \bf{69.05} \\
% German & 66.67 & \bf{75.00} & \textcolor{gray}{--} & 69.05 & 64.29 \\
% Spanish & \bf{77.38} & 73.81 & 75.00 & 76.19 & 72.62 \\
% Basque & 32.14 & 35.71 & \bf{36.90} & 33.33 & \bf{36.90} \\
% French & 61.90 & 67.86 & 64.29 & 67.86 & \bf{70.24} \\
% Galician & 64.29 & \bf{73.81} & 69.05 & 66.67 & \bf{73.81} \\
% Japanese & \bf{55.95} & \textcolor{gray}{--} & \bf{55.95} & \textcolor{gray}{--} & \textcolor{gray}{--} \\
% Russian & 71.43 & 69.05 & \bf{72.62} & \bf{72.62} & 69.05 \\
% Swahili & 55.95 & \bf{65.48} & 60.71 & 63.10 & \bf{65.48} \\
% Thai & 57.14 & \bf{61.90} & 54.76 & \bf{61.90} & 59.52 \\
% Chinese & 67.86 & \bf{71.43} & \bf{71.43} & \bf{71.43} & \bf{71.43} \\
% \midrule
% Average & 61.01 & \textbf{65.58} & 62.88 & 64.61 & 64.39 \\

% \bottomrule
% \end{tabular}
% \caption{Per-language accuracy results across different intervention points for the \llamamodel\ model on MGSM. Gray dashes indicate missing values. B = Baseline, OF = On Few-shot, AF = After Few-shot, OQ = On Question, ENT = Entire Prompt. \textbf{Bold} indicates the best score per language. German and Japanese did not have some configurations where validation set outperformed the baseline, hence, there are dashes.}
% \label{tab:intervention_detailed}
% \end{table}


\paragraph{Results on other Models.}
% Table~\ref{tab:main_results} summarizes average performance across all languages for each model--dataset combination. Overall, our method improves over the source baseline (B) in most settings, with particularly strong gains on MGSM across all three models. On MGSM, our method consistently outperforms the baseline, with improvements ranging from approximately 2.9\% to 5.4\%, indicating that activation steering is especially effective for structured mathematical reasoning tasks. 
% % Per-language results for \qwenseven\ and \qwenfourteen\ are provided in 
% % Appendix~\ref{app:other_models}.

% On XNLI and MSVAMP, improvements are generally smaller and more variable. Our method outperforms the baseline in several configurations, though the multilingual few-shot baseline (MFS) remains competitive and occasionally achieves higher accuracy, especially on MSVAMP. Despite this, our method performs comparably to or better than the baselines in the majority of cases,
% demonstrating that activation steering provides a consistent approach for improving cross-lingual transfer across the models and families tested. Qualitative examples illustrating the effect of steering on XNLI predictions 
% are provided in Appendix~\ref{app:qualitative}. Per-language results for \qwenseven\ and \qwenfourteen\ are in Appendix~\ref{app:other_models}; optimal layers and scaling factors in Appendix~\ref{appendix:hyperparams}; task-level configurations in Appendix~\ref{app:hparam}, which remain above the source baseline confirming the method is effective without per-language selection.

Table~\ref{tab:main_results} summarizes average performance across all languages for each model--dataset combination. Our method consistently outperforms the source baseline on MGSM across all three models, with improvements ranging from 2.9\% to 5.4\%, confirming that activation steering is especially effective for structured mathematical reasoning. On XNLI and MSVAMP, improvements are generally smaller, with MFS remaining competitive especially on MSVAMP. Despite this, our method performs comparably to or better than the baselines in the majority of cases across models and datasets. Per-language results for \qwenseven\ and \qwenfourteen\ are in Appendix~\ref{app:other_models}; optimal layers and scaling factors in Table \ref{tab:best_performing_layers}; for XNLI, layer 10 dominates across most languages, while earlier layers are more frequently optimal for MGSM and MSVAMP. Task-level configurations are in Appendix~\ref{app:hparam}, a single layer and scaling factor shared across all languages within a task remains consistently above the source baseline, confirming the method is effective without per-language selection as well.
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{6pt}
\small
\begin{tabular}{lccccclccccc}
\toprule
\multirow{2}{*}{Language} & \multicolumn{5}{c}{MGSM (vector) $\rightarrow$ XNLI (eval)} & & \multicolumn{5}{c}{XNLI (vector) $\rightarrow$ MGSM (eval)} \\
\cmidrule(lr){2-6} \cmidrule(lr){8-12}
 & B & MFS & Ours & CT & \cellcolor{LightGray!30}OR & & B & MFS & Ours & CT & \cellcolor{LightGray!30}OR \\
\midrule
Chinese & 78.14 & 77.84 & 77.84 & \bf{78.14} & \cellcolor{LightGray!30}79.34 & & 84.52 & 88.10 & 86.90 & \bf{90.48} & \cellcolor{LightGray!30}79.76 \\
Thai & 70.96 & \bf{73.05} & 70.06 & 70.06 & \cellcolor{LightGray!30}72.46 & & 79.76 & \bf{82.14} & 79.76 & \bf{82.14} & \cellcolor{LightGray!30}85.71 \\
Swahili & 53.29 & 47.31 & \bf{55.09} & 54.79 & \cellcolor{LightGray!30}54.79 & & 19.05 & 16.67 & \bf{26.19} & 25.00 & \cellcolor{LightGray!30}33.33 \\
Russian & 78.14 & 79.04 & \bf{79.64} & \bf{79.94} & \cellcolor{LightGray!30}78.74 & & 85.71 & 85.71 & \bf{88.10} & \bf{88.10} & \cellcolor{LightGray!30}85.71 \\
French & 81.44 & 82.34 & 82.34 & \bf{82.63} & \cellcolor{LightGray!30}82.63 & & 78.57 & 80.95 & \bf{79.76} & \bf{79.76} & \cellcolor{LightGray!30}84.52 \\
Spanish & 82.63 & 82.63 & \bf{83.53} & 83.23 & \cellcolor{LightGray!30}81.74 & & 84.52 & 83.33 & \bf{89.29} & 88.10 & \cellcolor{LightGray!30}86.90 \\
German & 81.74 & 77.54 & 82.93 & \bf{82.98} & \cellcolor{LightGray!30}79.34 & & 83.33 & 83.33 & \bf{85.71} & \bf{85.71} & \cellcolor{LightGray!30}86.90 \\
\midrule
Average & 75.19 & 74.22 & 75.92 & \bf{75.96} & \cellcolor{LightGray!30}75.58 & & 73.64 & 74.32 & \bf{76.53} & 76.36 & \cellcolor{LightGray!30}77.55 \\
\bottomrule
\end{tabular}



\begin{tabular}{lccccclccccc}
\toprule
\multirow{2}{*}{Language} 
& \multicolumn{5}{c}{MGSM (vector) $\rightarrow$ MSVAMP (eval)} 
& 
& \multicolumn{5}{c}{MSVAMP (vector) $\rightarrow$ MGSM (eval)} \\
\cmidrule(lr){2-6} \cmidrule(lr){8-12}
& B & MFS & Ours & CT & \cellcolor{LightGray!30}OR 
& 
& B & MFS & Ours & CT & \cellcolor{LightGray!30}OR \\
\midrule
Bengali  
& 65.57 & 70.96 & 67.07 & \bf{67.66} & \cellcolor{LightGray!30}76.35 
&& 58.33 & \bf{66.67} & 58.33 & 58.33 & \cellcolor{LightGray!30}65.48 \\

German   
& 79.04 & 79.94 & \bf{80.24} & 79.64 & \cellcolor{LightGray!30}81.14 
&& 83.33 & 83.33 & \bf{85.71} & 77.38 & \cellcolor{LightGray!30}86.90 \\

Spanish  
& 82.04 & 83.53 & \bf{83.83} & 82.04 & \cellcolor{LightGray!30}84.13 
&& 84.52 & 83.33 & 89.29 & \bf{90.48} & \cellcolor{LightGray!30}86.90 \\

French   
& 82.34 & \bf{85.03} & 84.13 & 79.04 & \cellcolor{LightGray!30}84.43 
&& 78.57 & \bf{80.95} & 79.76 & 77.38  & \cellcolor{LightGray!30}84.52 \\

Japanese 
& 78.74 & \bf{79.64} & \bf{79.64} & 79.34 & \cellcolor{LightGray!30}79.94 
&& 71.43 & 75.00 & 75.00 & \bf{76.19} & \cellcolor{LightGray!30}73.81 \\

Russian  
& 79.64 & \bf{82.93} & 81.74 & 80.54 & \cellcolor{LightGray!30}81.44 
&& 85.71 & 85.71 & \bf{88.10} & 83.33 & \cellcolor{LightGray!30}85.71 \\

Swahili 
& 49.10 & 47.90 & \bf{50.60} & 48.50 & \cellcolor{LightGray!30}50.30 
&& 19.05 & 16.67 & \bf{26.19} & 20.24 & \cellcolor{LightGray!30}33.33 \\

Thai    
& 78.14 & \bf{79.34} & \bf{79.34} & 76.65 & \cellcolor{LightGray!30}78.74 
&& 79.76 & 82.14 & \bf{86.90} & 78.57 & \cellcolor{LightGray!30}79.76 \\

Chinese 
& 82.04 & 83.23 & \bf{83.53} & 83.23 & \cellcolor{LightGray!30}82.34 
&& 84.52 & \bf{88.10} & 86.90 & \bf{88.10} & \cellcolor{LightGray!30}79.76 \\

\midrule
Average 
& 75.18 & \bf{76.94} & 76.68 & 75.18 & \cellcolor{LightGray!30}77.65 
&& 71.69 & 73.54 & \bf{74.34} & 72.22 & \cellcolor{LightGray!30} 75.79 \\
\bottomrule
\end{tabular}

\begin{tabular}{lccccclccccc}
\toprule
\multirow{2}{*}{Language} 
& \multicolumn{5}{c}{MSVAMP (vector) $\rightarrow$ XNLI (eval)} 
& 
& \multicolumn{5}{c}{XNLI (vector) $\rightarrow$ MSVAMP (eval)} \\
\cmidrule(lr){2-6} \cmidrule(lr){8-12}
& B & MFS & Ours & CT & \cellcolor{LightGray!30}OR 
& 
& B & MFS & Ours & CT & \cellcolor{LightGray!30}OR \\
\midrule
Chinese  
& 78.14 & \bf{77.84} & \bf{77.84} & 66.47 & \cellcolor{LightGray!30}79.34 
&& 82.04 & 83.23 & \bf{83.53} & 80.84 & \cellcolor{LightGray!30}82.34 \\

Thai    
& 70.96 & \bf{73.05} & 70.06 & 29.04 & \cellcolor{LightGray!30}72.46 
&& 78.14 & \bf{79.34} & \bf{79.34} & 76.35 & \cellcolor{LightGray!30}78.74 \\

Swahili 
& 53.29 & 47.31 & \bf{55.09} & 33.83 & \cellcolor{LightGray!30}54.79 
&& 49.10 & 47.90 & \bf{50.60} & 48.80 & \cellcolor{LightGray!30}50.30 \\

Russian  
& 78.14 & 79.04 & \bf{79.64} & 43.70 & \cellcolor{LightGray!30}78.74 
&& 79.64 & \bf{82.93} & 81.74 & 79.64 & \cellcolor{LightGray!30}81.44 \\

French   
& 81.44 & \bf{82.34} & \bf{82.34} & 50.60 & \cellcolor{LightGray!30}82.63 
&& 82.34 & \bf{85.03} & 84.13 & 81.44 & \cellcolor{LightGray!30}84.43 \\

Spanish  
& 82.63 & 82.63 & \bf{83.53} & 58.98 & \cellcolor{LightGray!30}81.74 
&& 82.04 & 83.53 & \bf{83.83} & 82.63 & \cellcolor{LightGray!30}84.13 \\

German   
& 81.74 & 77.54 & \bf{82.93} & 53.29 & \cellcolor{LightGray!30}79.34 
&& 79.04 & 79.94 & 80.24 & \bf{81.14} & \cellcolor{LightGray!30}81.14 \\

\midrule
Average 
& 75.19 & 74.22 & \bf{75.92} & 47.98 & \cellcolor{LightGray!30}75.58 
&& 75.18 & \bf{76.94} & 76.68  & 75.83 & \cellcolor{LightGray!30}77.65 \\
\bottomrule

\end{tabular}

\caption{ Cross-task transfer results across all task-vector combinations between MGSM, MSVAMP, and XNLI on \qwenseven. For each task pair, we compute steering vectors from one task and evaluate on another task. B = Baseline, MFS = Multilingual Few-Shot Baseline \cite{tu2025blessing}, CT = Cross-Transfer, OR = Oracle. Oracle is the upper bound and is not for a direct comparison. \textbf{Bold} indicates the best score.}
\label{tab:cross_task_detailed}
\end{table*}

Table~\ref{tab:intervention_detailed} shows accuracy across the four steering position configurations. On average, steering on the few-shot demonstrations (on\_fewshot) achieves the highest accuracy (65.58\%), roughly a $\sim$4 point improvement over baseline, though the best configuration remains language-dependent. In the absence of validation data, on\_fewshot is the recommended default. Having established that language vectors improve cross-lingual ICL performance, we now ask what these vectors actually encode, whether they capture language-specific structure or task-specific patterns, and whether that structure is linguistically meaningful.



% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{4pt}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% \multirow{2}{*}{Transfer Direction} & \multicolumn{5}{c}{Performance} \\
% \cmidrule(lr){2-6}
% & B & MFS & Ours & CT & \cellcolor{LightGray!30}OR \\
% \midrule
% MGSM $\rightarrow$ XNLI & 75.19 & 74.22 & \bf{75.92} & 75.96 & \cellcolor{LightGray!30}75.58 \\
% XNLI $\rightarrow$ MGSM & 73.64 & 74.32 & \bf{76.53} & 76.36 & \cellcolor{LightGray!30}77.55 \\
% MGSM $\rightarrow$ MSVAMP & 75.18 & \bf{76.94} & 76.68 & 75.18 & \cellcolor{LightGray!30}77.65 \\
% MSVAMP $\rightarrow$ MGSM & 71.69 & 73.54 & \bf{74.34} & 72.22 & \cellcolor{LightGray!30}75.79 \\
% XNLI $\rightarrow$ MSVAMP & 75.18 & \bf{76.94} & 76.68 & 75.83 & \cellcolor{LightGray!30}77.65 \\
% MSVAMP $\rightarrow$ XNLI & 75.19 & 74.22 & \bf{75.92} & 47.98 & \cellcolor{LightGray!30}75.58 \\
% \bottomrule
% \end{tabular}}
% \caption{Cross-task transfer results (averages) across all six transfer directions on \qwenseven. Vectors are computed from the source task and evaluated on the target task. B = Baseline, MFS = Multilingual Few-Shot Baseline \cite{tu2025blessing}, CT = Cross-Transfer, OR = Oracle. Oracle is the upper bound and is not for a direct comparison.}
% \label{tab:cross_task}
% \end{table}

% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{6pt}
% \resizebox{0.85\textwidth}{!}{
% \begin{tabular}{lccccclccccc}
% \toprule
% \multirow{2}{*}{Language} & \multicolumn{5}{c}{MGSM (vector) $\rightarrow$ XNLI (eval)} & & \multicolumn{5}{c}{XNLI (vector) $\rightarrow$ MGSM (eval)} \\
% \cmidrule(lr){2-6} \cmidrule(lr){8-12}
%  & B & MFS & Ours & CT & \cellcolor{LightGray!30}OR & & B & MFS & Ours & CT & \cellcolor{LightGray!30}OR \\
% \midrule
% Chinese & 78.14 & 77.84 & 77.84 & \bf{78.14} & \cellcolor{LightGray!30}79.34 & & 84.52 & 88.10 & 86.90 & \bf{90.48} & \cellcolor{LightGray!30}79.76 \\
% Thai & 70.96 & \bf{73.05} & 70.06 & 70.06 & \cellcolor{LightGray!30}72.46 & & 79.76 & \bf{82.14} & 79.76 & \bf{82.14} & \cellcolor{LightGray!30}85.71 \\
% Swahili & 53.29 & 47.31 & \bf{55.09} & 54.79 & \cellcolor{LightGray!30}54.79 & & 19.05 & 16.67 & \bf{26.19} & 25.00 & \cellcolor{LightGray!30}33.33 \\
% Russian & 78.14 & 79.04 & \bf{79.64} & \bf{79.94} & \cellcolor{LightGray!30}78.74 & & 85.71 & 85.71 & \bf{88.10} & \bf{88.10} & \cellcolor{LightGray!30}85.71 \\
% French & 81.44 & 82.34 & 82.34 & \bf{82.63} & \cellcolor{LightGray!30}82.63 & & 78.57 & 80.95 & \bf{79.76} & \bf{79.76} & \cellcolor{LightGray!30}84.52 \\
% Spanish & 82.63 & 82.63 & \bf{83.53} & 83.23 & \cellcolor{LightGray!30}81.74 & & 84.52 & 83.33 & \bf{89.29} & 88.10 & \cellcolor{LightGray!30}86.90 \\
% German & 81.74 & 77.54 & 82.93 & \bf{82.98} & \cellcolor{LightGray!30}79.34 & & 83.33 & 83.33 & \bf{85.71} & \bf{85.71} & \cellcolor{LightGray!30}86.90 \\
% \midrule
% Average & 75.19 & 74.22 & 75.92 & \bf{75.96} & \cellcolor{LightGray!30}75.58 & & 73.64 & 74.32 & \bf{76.53} & 76.36 & \cellcolor{LightGray!30}77.55 \\
% \bottomrule
% \end{tabular}}
% \caption{Cross-task transfer results for MGSM $\leftrightarrow$ XNLI on \qwenseven. B = Baseline, MFS = Multilingual Few-Shot Baseline \cite{tu2025blessing}, CT = Cross-Transfer, OR = Oracle (upper bound, not for direct comparison). \textbf{Bold} indicates the best score.}
% \label{tab:mgsm_xnli}
% \end{table*}



% demonstrating that activation steering provides a robust and model-agnostic approach for improving cross-lingual transfer across different model sizes and task types.


% The results are shown in \ref{tab:main_results} across all models and datasets. Detailed results for the XNLI dataset on the Llama3.1-8b-instruct model are shown in Table \ref{tab:xnli_detailed}. We see that our method consistently outperforms the baseline by an average of [insert percentage]. For the XNLI dataset, we see maximum gains

% If we look in detail at the XNLI results, we notice the following patterns: the strongest improvements are for the languages: Bulgarian, French, Russian and Vietnamese. Lesser gains are observed for Arabic, Thai and Chinese. On average, [method 2] outperforms the baseline and the blessing paper method.
